perf4sight: A toolflow to model CNN training performance on Edge GPUs

The increased memory and processing capabilities of today's edge devices create opportunities for greater edge intelligence. In the domain of vision, the ability to adapt a Convolutional Neural Network's (CNN) structure and parameters to the input data distribution leads to systems with lower memory footprint, latency and power consumption. However, due to the limited compute resources and memory budget on edge devices, it is necessary for the system to be able to predict the latency and memory footprint of the training process in order to identify favourable training configurations of the network topology and device combination for efficient network adaptation. This work proposes perf4sight, an automated methodology for developing accurate models that predict CNN training memory footprint and latency given a target device and network. This enables rapid identification of network topologies that can be retrained on the edge device with low resource consumption. With PyTorch as the framework and NVIDIA Jetson TX2 as the target device, the developed models predict training memory footprint and latency with 95% and 91% accuracy respectively for a wide range of networks, opening the path towards efficient network adaptation on edge GPUs.

==> figs/tex/model_construction.tex <==
\begin{figure*}[t!]
    \begin{tabular}{ccc}
        \subfloat[$mem_{used}$ for ResNet18 for various pruning levels]{
            \includegraphics[width = 0.3\textwidth]{figs/profiled_data/resnet18_mem_used.pdf} 
            \label{fig:resnet18_mem_used}
        } 
        \subfloat[Network-wise profiling process]{
            \includegraphics[trim={6.5cm 6.6cm 8.5cm 6cm},clip,width=0.3\textwidth]{figs/profiling_strat.pdf} 
            \label{fig:profiling_process}
        }
        \subfloat[Hierarchical training process]{
            \includegraphics[trim={10.8cm 3.8cm 11cm 3.3cm},clip,width=0.3\textwidth]{figs/toolflow_diagram.pdf} 
            \label{fig:toolflow}
        } 
    \end{tabular}
    \caption{}
    \label{}
\end{figure*}

==> figs/tex/oom_vary_mem.tex <==
\begin{figure}[t]
    \begin{minipage}[b]{\linewidth}
    \includegraphics[width = \textwidth]{figs/oom_vary_mem.pdf} 
    \caption{$oom$ test error rate when the $oom$ model was trained on data from the NVIDIA Jetson TX2 when all 8GB of memory was available and tested on data from environments limited to 4GB and 2GB memory}
    \label{fig:oom_vary_mem}
    \vspace{-0.3cm}
    \end{minipage}
\end{figure}

==> figs/tex/seen_basis.tex <==
\begin{figure*}[t!]
    \centering
    \begin{tabular}{cccc}
        \subfloat[Basis A]{\includegraphics[width = 0.25\textwidth]{figs/seen_basis/basis_A.pdf} \label{fig:seen_basis_a}}
        \subfloat[Basis B]{\includegraphics[width = 0.25\textwidth]{figs/seen_basis/basis_B.pdf} \label{fig:seen_basis_b}} 
        \subfloat[Basis C]{\includegraphics[width = 0.25\textwidth]{figs/seen_basis/basis_C.pdf} \label{fig:seen_basis_c}} 
        \subfloat[Basis D]{\includegraphics[width = 0.25\textwidth]{figs/seen_basis/basis_D.pdf} \label{fig:seen_basis_d}} 
        % \subfloat[Basis E]{\includegraphics[width = 0.3\textwidth]{figs/seen_basis/basis_E.pdf} \label{fig:seen_basis_e}} 
    \end{tabular}
    \caption{Performance of the basis model on networks present in the basis}
    \label{fig:seen_basis}
\end{figure*}

==> figs/tex/train_set_search.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width = 0.4\textwidth]{figs/train_set_search/search_results.pdf}
    \caption{Test error rates for training sets defined in Tab.\ref{tab:train_sets_searched}}
    \label{fig:train_set_search}
\end{figure}

==> figs/tex/unseen_basis.tex <==
\begin{figure*}[t!]
    \centering
    \begin{tabular}{cccc}
        \subfloat[Memory Allocated]{\includegraphics[width = 0.25\textwidth]{figs/unseen_basis/mem_alloc.pdf} \label{fig:unseen_basis_mem_alloc}}
        \subfloat[Memory Reserved]{\includegraphics[width = 0.25\textwidth]{figs/unseen_basis/mem_reserved.pdf} \label{fig:unseen_basis_mem_reserved}}
        \subfloat[Memory Used]{\includegraphics[width = 0.25\textwidth]{figs/unseen_basis/mem_used.pdf} \label{fig:unseen_basis_mem_used}}
        \subfloat[Latency]{\includegraphics[width = 0.25\textwidth]{figs/unseen_basis/latency.pdf} \label{fig:unseen_basis_latency}}
    \end{tabular}
    \caption{Performance of the basis model on networks not present in the basis}
    \label{fig:unseen_basis}
\end{figure*}

==> tables/attr_diffs.tex <==
\begin{table}[t]
    \begin{minipage}[b]{\linewidth}
    \begin{small}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|c}
            \toprule
            \multicolumn{7}{c}{\textbf{\textsc{Percentage Difference in Attribute Value (\%)}}} \\
            \cmidrule(lr){2-7}
            & \textit{ResNet18} & \textit{MobileNetV2} & \textit{SqueezeNet} & \textit{ResNet50} & \textit{MnasNet} & \textit{GoogLeNet} \\
            \midrule
            % $mem_{alloc}$ & 9.11 & 13.15 & 8.79 & 6.53 & 12.2 & 12.7\\
            % $mem_{reserved}$ & 11.7 & 13.1 & 12.0 & 5.82 & 12.8 & 14.0\\
            $\Gamma$ & 6.08 & 7.88 & 7.61 & 2.27 & 7.65 & 8.61 \\
            $\Phi$   & 8.59 & 12.7 & 10.1 & 6.83 & 11.5 & 12.6 \\
            \bottomrule
        \end{tabular}
    }
    \end{small}
    \caption{Upper bounds on acceptable mean attribute error rates ($\delta_{att}$) for a difference of 5pp ($r$) between pruning levels}
    \label{tab:attr_diffs}
    \vspace{-0.5cm}
    \end{minipage}
\end{table}


==> tables/basis_names.tex <==
\begin{table}[t]
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{cl}
            \toprule
            \multicolumn{1}{c}{\textbf{Basis Name}} &
            \multicolumn{1}{c}{\textbf{Networks}} &
            \midrule
            A & MnasNet, ResNet18, SqueezeNet \\
            B & MobileNetV2, ResNet50, GoogLeNet \\
            C & MnasNet, ResNet50, GoogLeNet \\
            D & MobileNetv2, ResNet18, SqueezeNet \\
            \bottomrule
        \end{tabular}}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
    \caption{Networks used as training data to form bases}
    \label{tab:basis}
\end{table}

==> tables/l1_prune_single_net.tex <==
\begin{table}[t]
    \vskip 0.15in
    \centering
    \begin{small}
    \begin{sc}
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{llllll}
        \toprule
        \multicolumn{2}{c}{\textbf{Network}} &
        \multicolumn{3}{c}{\textbf{Test Error Rates}} \\
        \cmidrule(lr){1-5}
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Train}}} &
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Test}}} &
        \multicolumn{3}{c}{\textbf{Memory}} \\
        % \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Latency}}} \\
        \cmidrule(lr){3-5}
        \multicolumn{1}{c}{\textbf{(Random)}} &
        \multicolumn{1}{c}{\textbf{(L1-Norm)}} &
        \multicolumn{1}{c}{\textbf{Allocated}} &
        \multicolumn{1}{c}{\textbf{Reserved}} &
        \multicolumn{1}{c}{\textbf{Used}} \\
        % \multicolumn{1}{c}{\textbf{}} \\
        \midrule
        MobileNetV2    & MobileNetV2    & 0.05 (0pp) & 0.04 (-3pp) & 0.05 (+1pp) \\ % & 0.07 \\
        ResNet18       & ResNet18       & 0.07 (+1pp) & 0.10 (0pp) & 0.06 (+1pp) \\ % & 0.05 
        SqueezeNet     & SqueezeNet     & 0.10 (+6pp) & 0.10 (+3pp) & 0.06 (+3pp) % & 0.05 
        % Basis 2 & MobileNetV2 (l1-norm)   & 0.04 & 0.03 & 0.05 \\ % & 0.07 \\
        % Basis 2 & ResNet18 (l1-norm)    & 0.08 & 0.10 & 0.06 \\ % & 0.05 
        % Basis 2 & SqueezeNet (l1-norm)    & 0.14 & 0.13 & 0.07 % & 0.05 
        \bottomrule
    \end{tabular}
    }
    \end{sc}
    \end{small}
    \vskip -0.1in
    \caption{Test error rates for memory prediction for networks trained on random pruning but tested on l1-pruning and difference in test error rates compared to a evaluation on a random pruning strategy (Tab.\ref{tab:single_network})}
    \label{tab:l1-norm-single-nets}
\end{table}

==> tables/linear_regressor.tex <==
\begin{table*}[t]
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lclcccc}
        \toprule
        \multicolumn{2}{c}{\textbf{Training}} & 
        \multicolumn{2}{c}{\textbf{Test}} & 
        \multicolumn{3}{c}{\textbf{Memory Prediction Error (\%)}} \\
        \midrule
        \textbf{Network}&
        \textbf{Pruning Levels (\%)} &
        \textbf{Network} &
        \textbf{Pruning Levels (\%)} &
        \textbf{Allocated} &
        \textbf{Reserved} &
        \textbf{Used} \\
        \midrule
        AlexNet     & 0 & AlexNet     & $\{5x \mid x \in {[}1,18{]}\}$ & 0.44 & 0.48 & 0.65 \\ 
        ResNet18    & 0 & ResNet18    & $\{5x \mid x \in {[}1,18{]}\}$ & 0.07 & 0.14 & 0.32 \\ 
        MobileNetV2 & 0 & MobileNetV2 & $\{5x \mid x \in {[}1,18{]}\}$ & 1.45 & 1.55 & 0.69 \\ 
        SqueezeNet  & 0 & SqueezeNet  & $\{5x \mid x \in {[}1,18{]}\}$ & 0.06 & 0.14 & 0.21 \\ 
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
    \caption{Memory allocated, reserved and used percentage prediction error for 4 networks using a linear regression model. }
    \label{tab:linear_regressor}
\end{table*}

==> tables/seen_basis.tex <==
\begin{table}[t]
    \vskip 0.15in
    \centering
    \begin{small}
    \begin{sc}
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{llcccc}
        \toprule
        \multicolumn{2}{c}{\textbf{Network}} &
        \multicolumn{4}{c}{\textbf{Test Error Rates}} \\
        \cmidrule(lr){1-6}
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Train}}} &
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Test}}} &
        \multicolumn{3}{c}{\textbf{Memory}} &
        \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Latency}}} \\
        \cmidrule(lr){3-5}
        \multicolumn{1}{c}{\textbf{(Random)}} &
        \multicolumn{1}{c}{\textbf{(Random)}} &
        \multicolumn{1}{c}{\textbf{Allocated}} &
        \multicolumn{1}{c}{\textbf{Reserved}} &
        \multicolumn{1}{c}{\textbf{Used}} &
        \multicolumn{1}{c}{\textbf{}} \\
        \midrule
        Basis A     & Basis A       & 0.07 & 0.09 & 0.04 & 0.06 \\
        Basis B     & Basis B       & 0.06 & 0.08 & 0.03 & 0.06 \\
        Basis C     & Basis C       & 0.05 & 0.07 & 0.03 & 0.06 \\
        Basis D     & Basis D       & 0.05 & 0.08 & 0.04 & 0.06 \\
        Basis E     & Basis E       & 0.04 & 0.05 & 0.03 & 0.05 \\
        \bottomrule
    \end{tabular}
    }
    \end{sc}
    \end{small}
    \vskip -0.1in
    \caption{Test error rates when training dataset includes multiple networks}
    \label{tab:single_network}
\end{table}

==> tables/single_net_unseen_pl.tex <==
% \begin{table*}[t]
%     \vskip 0.15in
%     \centering
%     \begin{small}
%     \begin{sc}
%     \begin{tabular}{llllcccc}
%         \toprule
%         \multicolumn{2}{c}{\textbf{Network}} &
%         \multicolumn{2}{c}{\textbf{Pruning Strategy}} &
%         \multicolumn{4}{c}{\textbf{Test Error (\%)}} \\
%         \cmidrule(lr){1-8}
%         \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Train}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Test}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Train}}} &
%         \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Test}}} &
%         \multicolumn{3}{c}{\textbf{Memory}} &
%         \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Latency}}} \\
%         \cmidrule(lr){5-7}
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{} &
%         \multicolumn{1}{c}{\textbf{Allocated}} &
%         \multicolumn{1}{c}{\textbf{Reserved}} &
%         \multicolumn{1}{c}{\textbf{Used}} &
%         \multicolumn{1}{c}{\textbf{}} \\
%         \midrule
%         ResNet18    & ResNet18      & Random    & Random    & 4.32 & 11.6 & 5.47 & 5.23 \\
%         \cite{resnet_He2016} &  &           & l1-norm   & 5.78  & 11.77 & 4.50 & 9.68 \\
%         \midrule
%         MobileNetV2 & MobileNetV2   & Random    & Random    & 1.57 & 3.54 & 1.52 & 6.52 \\
%         \cite{mobilenetv2_Sandler2018}  &       &   & l1-norm   & 4.12 & 3.46 & 3.22 & 6.01 \\
%         \midrule
%         SqueezeNet  & SqueezeNet    & Random    & Random    & 2.81 & 7.10 & 4.01 & 3.91 \\
%         \cite{squeezenet_Iandola2016}   &  &  & l1-norm   & 8.46 & 11.2 & 9.15 & 14.7 \\
%         \midrule
%         ResNet50    & ResNet50      & Random    & Random    & 2.98 & 5.01 & 1.93 & 3.03 \\
%         \cite{resnet_He2016}    & & & l1-norm & 4.91 & 5.33 & 3.12 & 6.19 \\
%         \midrule
%         MnasNet     & MnasNet       & Random    & Random    & 5.02 & 6.53 & 3.97 & 4.87 \\
%         \cite{mnasnet_Tan2018}  & & & l1-norm & 3.58 & 3.14 & 3.82 & 7.65 \\
%         \midrule
%         GoogLeNet   & GoogLeNet     & Random    & Random    & 2.03 & 3.87 & 1.71 & 4.54 \\
%         \cite{googlenet_Szegedy2015}  & & & l1-norm & 6.57 & 4.70 & 3.86 & 7.77\\
%         \bottomrule
%     \end{tabular}
%     \end{sc}
%     \end{small}
%     \vskip -0.1in
%     \caption{Test error rates for memory and latency prediction for training performed on profiled data for a single network.}
%     \label{tab:single_network}
% \end{table*}

\begin{table*}[t]
    \vskip 0.15in
    \centering
    \begin{small}
    \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
        \toprule
        \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\textsc{Attribute}}}} &
        \multicolumn{12}{c}{\textbf{\textsc{Test Error (\%)}}} \\
        \cmidrule(lr){2-13}
        \multicolumn{1}{c|}{} &
        \multicolumn{2}{c|}{{\textit{ResNet18} \cite{resnet_He2016}}} &
        \multicolumn{2}{c|}{{\textit{MobileNetV2} \cite{mobilenetv2_Sandler2018}}} &
        \multicolumn{2}{c|}{{\textit{SqueezeNet} \cite{squeezenet_Iandola2016}}} &
        \multicolumn{2}{c|}{{\textit{ResNet50}}} &
        \multicolumn{2}{c|}{{\textit{MnasNet} \cite{mnasnet_Tan2018}}} &
        \multicolumn{2}{c}{{\textit{GoogLeNet} \cite{googlenet_Szegedy2015}}} \\
        \multicolumn{1}{c|}{} &
        \multicolumn{1}{c}{{Rand}} & 
        \multicolumn{1}{c|}{{L1}} & 
        \multicolumn{1}{c}{{Rand}} & 
        \multicolumn{1}{c|}{{L1}} & 
        \multicolumn{1}{c}{{Rand}} & 
        \multicolumn{1}{c|}{{L1}} & 
        \multicolumn{1}{c}{{Rand}} & 
        \multicolumn{1}{c|}{{L1}} & 
        \multicolumn{1}{c}{{Rand}} & 
        \multicolumn{1}{c|}{{L1}} & 
        \multicolumn{1}{c}{{Rand}} & 
        \multicolumn{1}{c}{{L1}} \\
        \midrule
        $mem_{alloc}$ & 4.32 & 5.78 & 1.57 & 4.12 & 2.81 & 8.46 & 2.98 & 4.91 & 5.02 & 3.58 & 2.03 & 6.57 \\
        $mem_{reserved}$ & 11.6 & 11.77 & 3.54 & 3.46 & 7.10 & 11.2 & 5.01 & 5.33 & 6.53 & 3.14 & 3.87 & 4.70 \\
        $mem_{used}$ & 5.47 & 4.50 & 1.52 & 3.22 & 4.01 & 9.15 & 1.93 & 3.12 & 3.97 & 3.82 & 1.71 & 3.86 \\
        $latency$ & 5.23 & 9.68 & 6.52 & 6.01 & 3.91 & 14.7 & 3.03 & 6.19 & 4.87 & 7.65 & 4.54 & 7.77 \\
        $oom$ & 8.60 & 8.65 & 1.76 & 1.47 & 3.43 & 6.13 & 3.19 & 4.32 & 2.45 & 5.24 & 2.37 & 9.27          \\
        \bottomrule
    \end{tabular}
    \end{small}
    \vskip -0.1in
    \caption{Mean test error of memory and latency prediction across all batch sizes and pruning levels on uniform randomly pruned and L1-norm pruned networks. Batch sizes profiled were \{2,4,8,16,32,64,80,90,100,110,128,140,150,160,170,180,190,200,210,220,230,240,256\} and pruning levels in the test set were \{$5x | x \in [0,18], x \notin \{0,30,50,70,90\}$\}}.
    \label{tab:single_network}
\end{table*}

==> tables/train_set_size.tex <==
\begin{table}[t]
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \resizebox{0.5\textwidth}{!}{
        \begin{tabular}{cl}
            \toprule
            \textbf{Train Set Index} &
            \textbf{Train Set Pruning Levels (\%)} &
            \midrule
            A & $T = \{{0}\}$ \\
            B & $T = \{{0,90}\}$ \\
            C & $T = \{{0,50,90}\}$ \\
            D & $T = \{{0,50,70,90}\}$ \\
            E & $T = \{{0,30,50,90}\}$ \\
            F & $T = \{{0,30,50,70,90}\}$ \\
            G & $T = \{{0,20,30,50,70,90}\}$ \\
            H & $T = \{{0,20,30,50,60,70,90}\}$ \\
            I & $T = \{{0,10,20,30,50,60,70,90}\}$ \\
            \bottomrule
        \end{tabular}
    }
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
    \caption{Pruning levels used in various training sets}
    \label{tab:train_sets_searched}
\end{table}
